Socializing the Semantic Gap: A Comparative Survey on Image Tag Assignment, Refinement and Retrieval

Where previous reviews on content-based image retrieval emphasize on what can be seen in an image to bridge the semantic gap, this survey considers what people tag about an image. A comprehensive treatise of three closely linked problems, i.e., image tag assignment, refinement, and tag-based image retrieval is presented. While existing works vary in terms of their targeted tasks and methodology, they rely on the key functionality of tag relevance, i.e. estimating the relevance of a specific tag with respect to the visual content of a given image and its social context. By analyzing what information a specific method exploits to construct its tag relevance function and how such information is exploited, this paper introduces a taxonomy to structure the growing literature, understand the ingredients of the main works, clarify their connections and difference, and recognize their merits and limitations. For a head-to-head comparison between the state-of-the-art, a new experimental protocol is presented, with training sets containing 10k, 100k and 1m images and an evaluation on three test sets, contributed by various research groups. Eleven representative works are implemented and evaluated. Putting all this together, the survey aims to provide an overview of the past and foster progress for the near future.

==> future.tex <==
\subsection{Reflection and future work}

Much progress has been made. 
Given the current test tag set, the best-performing methods already outperform social tagging for tag assignment (MiAP of 0.392 versus 0.204 on MIRFlickr and 0.396 versus 0.255 on NUS-WIDE). Image retrieval using learned tag relevance also yields more accurate results compared to image retrieval using original tags (MAP of 0.881 versus 0.595 on Flickr55 and 0.738 versus 0.489 on NUS-WIDE). For tag assignment and tag retrieval, methods that exploit tag + image media by instance-based learning take the leading position.  
Methods that exploit tag + image + user information by transduction-based learning are more suited for tag refinement. 
These baselines need to be compared against when one advocates a new method.

Much remains to be done. Several exciting recent developments open up new opportunities for the future.  
First, employing novel deep learning based visual features is likely to boost the performance of the tag + image based methods.  What is scientifically more interesting is to devise a learning strategy that is capable of jointly exploiting tag, image, and user information in a much more scalable manner than currently feasible. 
The importance of the filter component, which refines socially tagged training examples in advance to learning, is underestimated.  
As denoising often comes with the price of reducing visual diversity, more research attention is required to understand what an acceptable level of noise shall be for learning tag relevance. 
Having a number of collaboratively labeled resources publicly available, e.g., ImageNet as a profound example, research on joint exploration of social data and these resources is important.
This connects to the most fundamental aspect of content-based image retrieval in the context of sharing and tagging within social media platforms: to what extent a social tag can be trusted remains open.  
Image retrieval by multi-tag query is another important yet largely unexplored problem.  For a query of two tags, it is suggested to view the two tags as a single bi-gram tag \cite{tmm12-li,mm2012-nie,mm2013-borth}, which is found to be superior to late fusion of individual tag scores.  Nonetheless, due to the increasing sparseness of n-grams, how to effectively answer generic queries of more than two tag is challenging. 
Moreover, test tags in the current benchmark sets were picked based on availability. 
It would be relevant to investigate why people search images on social media platforms and what query terms they use. 
We have not seen any quantitative study in this direction. 
Although some query log data of generic web image search has been publicly accessible \cite{mm2013-hua}, its social-media counterpart remains to be established. 
Last but not least, fine-grained ground truth that enables us to evaluate various tag relevance learning methods for answering ambiguous tags is currently missing.

